Stein Variational Gradient Descent: A General Purpose Bayesian Inference Algorithm

We propose a general purpose variational inference algorithm that forms a natural counterpart of gradient descent for optimization. Our method iteratively transports a set of particles to match the target distribution, by applying a form of functional gradient descent that minimizes the KL divergence. Empirical studies are performed on various real world models and datasets, on which our method is competitive with existing state-of-the-art methods. The derivation of our method is based on a new theoretical result that connects the derivative of KL divergence under smooth transforms with Stein's identity and a recently proposed kernelized Stein discrepancy, which is of independent interest.

==> bak <==
@article{oates2014control,
  title={Control functionals for Monte Carlo integration},
  author={Oates, Chris J and Girolami, Mark and Chopin, Nicolas},
  journal={Journal of the Royal Statistical Society, Series B},
  year={2017}
}

@article{chwialkowski2016kernel,
  title={A Kernel Test of Goodness of Fit},
  author={Chwialkowski, Kacper and Strathmann, Heiko and Gretton, Arthur},
  journal={ICML},
  year={2016}
}


@article{zhou2008derivative,
  title={Derivative reproducing properties for kernel methods in learning theory},
  author={Zhou, Ding-Xuan},
  journal={Journal of computational and Applied Mathematics},
  volume={220},
  number={1},
  pages={456--463},
  year={2008},
  publisher={Elsevier}
}

@article{gretton2012kernel,
  title={A kernel two-sample test},
  author={Gretton, Arthur and Borgwardt, Karsten M and Rasch, Malte J and Sch{\"o}lkopf, Bernhard and Smola, Alexander},
  journal={The Journal of Machine Learning Research},
  volume={13},
  number={1},
  pages={723--773},
  year={2012},
  publisher={JMLR. org}
}

@article{ley2013stein,
  title={Stein's density approach and information inequalities},
  author={Ley, Christophe and Swan, Yvik},
  journal={Electron. Comm. Probab},
  volume={18},
  number={7},
  pages={1--14},
  year={2013}
}


@inproceedings{peel2010empirical,
  title={Empirical Bernstein inequalities for u-statistics},
  author={Peel, Thomas and Anthoine, Sandrine and Ralaivola, Liva},
  fullbooktitle={Advances in Neural Information Processing Systems},
  booktitle={NIPS},    
  pages={1903--1911},
  year={2010}
}


@article{nguyen2010estimating,
  title={Estimating divergence functionals and the likelihood ratio by convex risk minimization},
  author={Nguyen, XuanLong and Wainwright, Martin J and Jordan, Michael and others},
  journal={Information Theory, IEEE Transactions on},
  volume={56},
  number={11},
  pages={5847--5861},
  year={2010},
  publisher={IEEE}
}

@inproceedings{lyu2009interpretation,
  title={Interpretation and generalization of score matching},
  author={Lyu, Siwei},
  _booktitle={Proceedings of the Twenty-Fifth Conference on Uncertainty in Artificial Intelligence},
  fullbooktitle={Conference on Uncertainty in Artificial Intelligence (UAI)},  
  booktitle = {UAI},
  pages={359--366},
  year={2009},
  _organization={AUAI Press}
}

@inproceedings{goyal2014fourier,
  title={Fourier PCA and robust tensor decomposition},
  author={Goyal, Navin and Vempala, Santosh and Xiao, Ying},
  booktitle={Proceedings of the 46th Annual ACM Symposium on Theory of Computing},
  pages={584--593},
  year={2014},
  organization={ACM}
}

@article{anandkumar2012method,
  title={A method of moments for mixture models and hidden Markov models},
  author={Anandkumar, Animashree and Hsu, Daniel and Kakade, Sham M},
  journal={arXiv preprint arXiv:1203.0683},
  year={2012}
}

@inproceedings{welling2004exponential,
  title={Exponential family harmoniums with an application to information retrieval},
  author={Welling, Max and Rosen-Zvi, Michal and Hinton, Geoffrey E},
  booktitle={Advances in neural information processing systems},
  pages={1481--1488},
  year={2004}
}

@article{zhang2015ell_1,
  title={$$\backslash$ ell\_1 $-regularized Neural Networks are Improperly Learnable in Polynomial Time},
  author={Zhang, Yuchen and Lee, Jason D and Jordan, Michael I},
  journal={arXiv preprint arXiv:1510.03528},
  year={2015}
}

@article{janzamin2015beating,
  title={Beating the Perils of Non-Convexity: Guaranteed Training of Neural Networks using Tensor Methods},
  author={Janzamin, Majid and Sedghi, Hanie and Anandkumar, Anima},
  journal={CoRR abs/1506.08473},
  year={2015}
}


@article{birge1995estimation,
  title={Estimation of integral functionals of a density},
  author={Birge, Lucien and Massart, Pascal},
  journal={The Annals of Statistics},
  pages={11--29},
  year={1995},
  publisher={JSTOR}
}

@article{laurent1996efficient,
  title={Efficient estimation of integral functionals of a density},
  author={Laurent, B{\'e}atrice and others},
  journal={The Annals of Statistics},
  volume={24},
  number={2},
  pages={659--681},
  year={1996},
  publisher={Institute of Mathematical Statistics}
}

@article{kerkyacharian1996estimating,
  title={Estimating nonquadratic functionals of a density using Haar wavelets},
  author={Kerkyacharian, G{\'e}rard and Picard, Dominique and others},
  journal={The Annals of Statistics},
  volume={24},
  number={2},
  pages={485--507},
  year={1996},
  publisher={Institute of Mathematical Statistics}
}


@inproceedings{Krishnamurthynips15,
  title={Influence Functions for Machine Learning: Nonparametric Estimators for Entropies, Divergences, and Mutual Informations},
  author={Kirthevasan Kandasamy and Akshay Krishnamurthy and Barnabas Poczos and Larry Wasserman and James M. Robins}, 
  fullbooktitle={Neural Information Processing Systems (NIPS)},
  booktitle={NIPS},  
  year={2015}
}

@inproceedings{Krishnamurthyaistats15,
title = {On Estimating $L_2^2$ Divergence},   
author={Akshay Krishnamurthy and Kirthevasan Kandasamy and Barnabas Poczos and Larry Wasserman},
booktitle = {Artificial Intelligence and Statistics (AISTATS)},
year = { 2015}
}

@inproceedings{Krishnamurthyicml15,
author = {Akshay Krishnamurthy and Kirthevasan Kandasamy and Barnabas Poczos, and Larry Wasserman},
title = {Nonparametric Estimation of {Renyi} Divergence and Friends},
booktitle = { ICML},
year =  {2014}
}


@book{steinwart2008support,
  title={Support vector machines},
  author={Steinwart, Ingo and Christmann, Andreas},
  year={2008},
  publisher={Springer Science \& Business Media}
}

@article{zhou2008derivative,
  title={Derivative reproducing properties for kernel methods in learning theory},
  author={Zhou, Ding-Xuan},
  journal={Journal of computational and Applied Mathematics},
  volume={220},
  number={1},
  pages={456--463},
  year={2008},
  publisher={Elsevier}
}

@article{hoeffding1948class,
  title={A class of statistics with asymptotically normal distribution},
  author={Hoeffding, Wassily},
  journal={The annals of mathematical statistics},
  pages={293--325},
  year={1948},
  publisher={JSTOR}
}


@article{arcones1995bernstein,
  title={A Bernstein-type inequality for {U}-statistics and {U}-processes},
  author={Arcones, Miguel A},
  journal={Statistics \& probability letters},
  volume={22},
  number={3},
  pages={239--247},
  year={1995},
  publisher={Elsevier}
}

@article{hoeffding1963probability,
  title={Probability inequalities for sums of bounded random variables},
  author={Hoeffding, Wassily},
  journal={Journal of the American statistical association},
  volume={58},
  number={301},
  pages={13--30},
  year={1963},
  publisher={Taylor \& Francis Group}
}

@inproceedings{peel2010empirical,
  title={Empirical Bernstein inequalities for {U}-statistics},
  author={Peel, Thomas and Anthoine, Sandrine and Ralaivola, Liva},
  fullbooktitle={Advances in Neural Information Processing Systems},
  booktitle = {NIPS},
  pages={1903--1911},
  year={2010}
}

@article{grimmett1992probability,
  title={Probability and random processes},
  author={Grimmett, Geoffrey and Stirzaker, David},
  year={1992}
}

@article{mason1992rank,
  title={A rank statistics approach to the consistency of a general bootstrap},
  author={Mason, David M and Newton, Michael A},
  journal={The Annals of Statistics},
  pages={1611--1624},
  year={1992},
  publisher={JSTOR}
}

@article{huskova1993consistency,
  title={Consistency of the generalized bootstrap for degenerate {U}-statistics},
  author={Huskova, Marie and Janssen, Paul},
  journal={The Annals of Statistics},
  pages={1811--1823},
  year={1993},
  publisher={JSTOR}
}

@article{arcones1992bootstrap,
  title={On the bootstrap of {U} and {V} statistics},
  author={Arcones, Miguel A and Gine, Evarist},
  journal={The Annals of Statistics},
  pages={655--674},
  year={1992},
  publisher={JSTOR}
}




@article{ho2006two,
  title={Two-stage {U}-statistics for Hypothesis Testing},
  _author={HO, HWAI-CHUNG and Shieh, Grace S},
    author={Ho, Hwai-Chung and Shieh, Grace S},
  journal={Scandinavian journal of statistics},
  volume={33},
  number={4},
  pages={861--873},
  year={2006},
  publisher={Wiley Online Library}
}

@inproceedings{gretton2009fast,
  title={A fast, consistent kernel two-sample test},
  author={Gretton, Arthur and Fukumizu, Kenji and Harchaoui, Zaid and Sriperumbudur, Bharath K},
  booktitle={Advances in neural information processing systems},
  pages={673--681},
  year={2009}
}

@inproceedings{stein1972,
_address = "Berkeley, Calif.",
author = "Stein, Charles",
booktitle = "Proceedings of the Sixth Berkeley Symposium on Mathematical Statistics and Probability, Volume 2: Probability Theory",
pages = "583--602",
_publisher = "University of California Press",
title = "A bound for the error in the normal approximation to the distribution of a sum of dependent random variables",
_url = "http://projecteuclid.org/euclid.bsmsp/1200514239",
year = "1972"
}


@article{chatterjee2007stein,
  title={Stein's method for concentration inequalities},
  author={Chatterjee, Sourav},
  journal={Probability theory and related fields},
  volume={138},
  number={1},
  pages={305--321},
  year={2007},
  publisher={Springer}
}

@book{barbour2005introduction,
  title={An introduction to Stein's method},
  author={Barbour, Andrew D and Chen, Louis Hsiao Yun},
  volume={4},
  year={2005},
  publisher={World Scientific}
}

@book{stein2005stein,
  title={Stein's Method and Applications},
  author={Stein, Charles and Barbour, Andrew D and Chen, Louis Hsiao Yun},
  volume={5},
  year={2005},
  publisher={World Scientific}
}

@article{reinert2005three,
  title={Three general approaches to Stein?s method},
  author={Reinert, Gesine},
  journal={An introduction to Stein?s method},
  volume={4},
  pages={183--221},
  year={2005},
  publisher={World Scientific}
}

@article{hoeffding1948class,
  title={A class of statistics with asymptotically normal distribution},
  author={Hoeffding, Wassily},
  journal={The annals of mathematical statistics},
  pages={293--325},
  year={1948},
  publisher={JSTOR}
}

@book{serfling2009approximation,
  title={Approximation theorems of mathematical statistics},
  author={Serfling, Robert J},
  volume={162},
  year={2009},
  publisher={John Wiley \& Sons}
}

@article{grosse2015sandwiching,
  title={Sandwiching the marginal likelihood using bidirectional Monte Carlo},
  author={Grosse, Roger B and Ghahramani, Zoubin and Adams, Ryan P},
  journal={arXiv preprint arXiv:1511.02543},
  year={2015}
}

@article{gelfand1994bayesian,
  title={Bayesian model choice: asymptotics and exact calculations},
  author={Gelfand, Alan E and Dey, Dipak K},
  journal={Journal of the Royal Statistical Society. Series B (Methodological)},
  pages={501--514},
  year={1994},
  publisher={JSTOR}
}

@inproceedings{salakhutdinov2008quantitative,
  title={On the quantitative analysis of deep belief networks},
  author={Salakhutdinov, Ruslan and Murray, Iain},
  fullbooktitle={Proceedings of the 25th international conference on Machine learning},
  booktitle={ICML},  
  pages={872--879},
  year={2008},
  _organization={ACM}
}

@inproceedings{burda2015accurate,
  title={$\{$Accurate and conservative estimates of MRF log-likelihood using reverse annealing$\}$},
  author={Burda, Yuri and Grosse, Roger and Salakhutdinov, Ruslan},
  booktitle={Proceedings of the Eighteenth International Conference on Artificial Intelligence and Statistics},
  pages={102--110},
  year={2015}
}


@article{neyman1937smooth,
  title={Smooth test for goodness of fit},
  author={Neyman, Jerzy},
  journal={Scandinavian Actuarial Journal},
  volume={1937},
  number={3-4},
  pages={149--199},
  year={1937},
  publisher={Taylor \& Francis}
}


@inproceedings{liuuai15,
author = {Q. Liu and J. Peng and A. Ihler and J. Fisher III},
title = {Estimating the Partition Function by Discriminance Sampling},
booktitle={UAI },
_booktitle = "Proceedings of the 31st Conference Annual Conference on Uncertainty in Artificial Intelligence (UAI-15)",
_publisher = "AUAI Press",
year = "2015",
}


@inproceedings{gretton2006kernel,
  title={A kernel method for the two-sample-problem},
  author={Gretton, Arthur and Borgwardt, Karsten M and Rasch, Malte and Sch{\"o}lkopf, Bernhard and Smola, Alex J},
  booktitle={Advances in neural information processing systems},
  pages={513--520},
  year={2006}
}


@article{ledwina1994data,
  title={Data-driven version of Neyman's smooth test of fit},
  author={Ledwina, Teresa},
  journal={Journal of the American Statistical Association},
  volume={89},
  number={427},
  pages={1000--1005},
  year={1994},
  publisher={Taylor \& Francis Group}
}

@article{fan1996test,
 ISSN = {01621459},
 URL = {http://www.jstor.org/stable/2291663},
 author = {Jianqing Fan},
 journal = {Journal of the American Statistical Association},
 number = {434},
 pages = {674-688},
 publisher = {Taylor & Francis, Ltd.},
 title = {Test of Significance Based on Wavelet Thresholding and Neyman's Truncation},
 volume = {91},
 year = {1996}
}



@book{lehmann2006testing,
  title={Testing statistical hypotheses},
  author={Lehmann, Erich L and Romano, Joseph P},
  year={2006},
  publisher={Springer Science \& Business Media}
}


@article{hall1987estimation,
  title={Estimation of integrated squared density derivatives},
  author={Hall, Peter and Marron, James Stephen},
  journal={Statistics \& Probability Letters},
  volume={6},
  number={2},
  pages={109--115},
  year={1987},
  publisher={Elsevier}
}

@book{zayed1996handbook,
  title={Handbook of function and generalized function transformations},
  author={Zayed, Ahmed I},
  year={1996},
  publisher={CRC press}
}


@incollection{stein2004use,
  title={Use of exchangeable pairs in the analysis of simulations},
  author={Stein, Charles and Diaconis, Persi and Holmes, Susan and Reinert, Gesine and others},
  booktitle={Stein's Method},
  pages={1--25},
  year={2004},
  publisher={Institute of Mathematical Statistics}
}

@article{sriperumbudur2013density,
  title={Density estimation in infinite dimensional exponential families},
  author={Sriperumbudur, Bharath and Fukumizu, Kenji and Kumar, Revant and Gretton, Arthur and Hyv{\"a}rinen, Aapo},
  journal={arXiv preprint arXiv:1312.3516},
  year={2013}
}

@book{marsden2003vector,
  title={Vector calculus},
  author={Marsden, Jerrold Eldon and Tromba, Anthony},
  year={2003},
  publisher={Macmillan}
}

@incollection{chandrasekaran2008complexity,
_author = {V. Chandrasekaran and N. Srebro and P. Harsha},
  author={Chandrasekaran, Venkat and Srebro, Nathan and Harsha, Prahladh},
title = {Complexity of Inference in Graphical Models},
fullbooktitle  = {Conference on Uncertainty in Artificial Intelligence and Statistics (UAI)},
 booktitle = {UAI},
month = {July},
year = {2008}
}



@inproceedings{hyvarinen2005estimation,
  title={Estimation of non-normalized statistical models by score matching},
  author={Hyv{\"a}rinen, Aapo},
  booktitle={Journal of Machine Learning Research},
  pages={695--709},
  year={2005}
}

@article{neal2001annealed,
  title={Annealed importance sampling},
  author={Neal, Radford M},
  journal={Statistics and Computing},
  volume={11},
  number={2},
  pages={125--139},
  year={2001},
  publisher={Springer}
}

@book{koller2009probabilistic,
  title={Probabilistic graphical models: principles and techniques},
  author={Koller, Daphne and Friedman, Nir},
  year={2009},
  publisher={MIT press}
}

@article{ruslan,
author = {Ruslan Salakhutdinov},
title = {Learning Deep Generative Models},
journal = {Annual Review of Statistics and Its Application},
volume = {2},
number = {1},
pages = {361-385},
year = {2015}
}


@inproceedings{gorham2015measuring,
  title={Measuring Sample Quality with Stein's Method},
  author={Gorham, Jack and Mackey, Lester},
  fullbooktitle={Advances in Neural Information Processing Systems},
  booktitle={NIPS},  
  pages={226--234},
  year={2015}
}

@inproceedings{Zaremba2013b,
title = { B-tests: Low Variance Kernel Two-Sample Tests},
author = {Zaremba, Wojciech and Gretton, Arthur and Blaschko, Matthew B.},
fullbooktitle = {Advances in Neural Information Processing Systems},
booktitle = {NIPS},
_editor = {C.J.C. Burges and L. Bottou and M. Welling and Z. Ghahramani and K.Q. Weinberger},
pages = {755--763},
year = {2013},
_publisher = {Curran Associates, Inc.},
}


@inproceedings{welling2004exponential,
  title={Exponential family harmoniums with an application to information retrieval},
  author={Welling, Max and Rosen-Zvi, Michal and Hinton, Geoffrey E},
  booktitle={NIPS},  
 fullbooktitle={Advances in neural information processing systems},
  pages={1481--1488},
  year={2004}
}

@article{hinton2006reducing,
  title={Reducing the dimensionality of data with neural networks},
  author={Hinton, Geoffrey E and Salakhutdinov, Ruslan R},
  journal={Science},
  volume={313},
  number={5786},
  pages={504--507},
  year={2006},
  publisher={American Association for the Advancement of Science}
}

@book{d1986goodness,
  title={Goodness-of-fit-techniques},
  author={D'Agostino, Ralph B},
  volume={68},
  year={1986},
  publisher={CRC press}
}

@book{chen2012monte,
  title={Monte Carlo methods in Bayesian computation},
  author={Chen, Ming-Hui and Shao, Qi-Man and Ibrahim, Joseph G},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@inproceedings{chwialkowski2014wild,
  title={A wild bootstrap for degenerate kernel tests},
  author={Chwialkowski, Kacper P and Sejdinovic, Dino and Gretton, Arthur},
  booktitle={Advances in neural information processing systems},
  pages={3608--3616},
  year={2014}
}

@book{johnson2004information,
  title={Information theory and the central limit theorem},
  author={Johnson, Oliver},
  volume={8},
  year={2004},
  publisher={World Scientific}
}

@article{oates2016convergence,
  title={Convergence Rates for a Class of Estimators Based on Stein's Identity},
  author={Oates, Chris J and Cockayne, Jon and Briol, Fran{\c{c}}ois-Xavier and Girolami, Mark},
  journal={arXiv preprint arXiv:1603.03220},
  year={2016}
}

@inproceedings{li2015toward,
  title={Toward Minimax Off-policy Value Estimation.},
  author={Li, Lihong and Munos, R{\'e}mi and Szepesv{\'a}ri, Csaba},
  booktitle={AISTATS},
  year={2015}
}

@article{hirano2003efficient,
  title={Efficient estimation of average treatment effects using the estimated propensity score},
  author={Hirano, Keisuke and Imbens, Guido W and Ridder, Geert},
  journal={Econometrica},
  volume={71},
  number={4},
  pages={1161--1189},
  year={2003},
  publisher={Wiley Online Library}
}


@article{henmi2007importance,
  title={Importance sampling via the estimated sampler},
  author={Henmi, Masayuki and Yoshida, Ryo and Eguchi, Shinto},
  journal={Biometrika},
  volume={94},
  number={4},
  pages={985--991},
  year={2007},
  publisher={Biometrika Trust}
}


@book{niederreiter2010quasi,
  title={Quasi-Monte Carlo Methods},
  author={Niederreiter, Harald},
  year={2010},
  publisher={Wiley Online Library}
}

@inproceedings{ghahramani2002bayesian,
  title={Bayesian monte carlo},
  author={Ghahramani, Zoubin and Rasmussen, Carl E},
  booktitle={Advances in neural information processing systems},
  pages={489--496},
  year={2002}
}

@article{briol2015probabilistic,
  title={Probabilistic Integration},
  author={Briol, Fran{\c{c}}ois-Xavier and Oates, Chris and Girolami, Mark and Osborne, Michael A and Sejdinovic, Dino and others},
  journal={arXiv preprint arXiv:1512.00933},
  year={2015}
}

@inproceedings{chen2010super,
author = {Yutian Chen and Max Welling and Alex Smola}, 
title = {Super-Samples from Kernel Herding},
booktitle = {Conference on Uncertainty in Artificial Intelligence (UAI)}, 
year = {2010}
}

@article{bach2015equivalence,
  title={On the equivalence between quadrature rules and random features},
  author={Bach, Francis},
  journal={arXiv preprint arXiv:1502.06800},
  year={2015}
}


@article{o1991bayes,
  title={Bayes--hermite quadrature},
  author={O'Hagan, Anthony},
  journal={Journal of statistical planning and inference},
  volume={29},
  number={3},
  pages={245--260},
  year={1991},
  publisher={Elsevier}
}

@inproceedings{liu2016kernelized,
  title={A Kernelized Stein Discrepancy for Goodness-of-fit Tests and Model Evaluation},
  author={Liu, Qiang and Lee, Jason D and Jordan, Michael I},
  booktitle={ICML (to appear)},
  year={2016}
}

@article{chwialkowski2016kernel,
  title={A Kernel Test of Goodness of Fit},
  author={Chwialkowski, Kacper and Strathmann, Heiko and Gretton, Arthur},
  journal={arXiv preprint arXiv:1602.02964},
  year={2016}
}

@book{scholkopf2001learning,
  title={Learning with kernels: support vector machines, regularization, optimization, and beyond},
  author={Scholkopf, Bernhard and Smola, Alexander J},
  year={2001},
  publisher={MIT press}
}

@inproceedings{smola2007hilbert,
  title={A Hilbert space embedding for distributions},
  author={Smola, Alex and Gretton, Arthur and Song, Le and Sch{\"o}lkopf, Bernhard},
  booktitle={Algorithmic learning theory},
  pages={13--31},
  year={2007},
  organization={Springer}
}

@book{robert2013monte,
  title={Monte Carlo statistical methods},
  author={Robert, Christian and Casella, George},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@article{neal2001annealed,
  title={Annealed importance sampling},
  author={Neal, Radford M},
  journal={Statistics and Computing},
  volume={11},
  number={2},
  pages={125--139},
  year={2001},
  publisher={Springer}
}
@book{smith2013sequential,
  title={Sequential Monte Carlo methods in practice},
  author={Smith, Adrian and Doucet, Arnaud and de Freitas, Nando and Gordon, Neil},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@article{kawakita2012semi,
  title={Semi-Supervised learning with Density-Ratio Estimation},
  author={Kawakita, Masanori and Kanamori, Takafumi},
  journal={arXiv preprint arXiv:1204.3965},
  year={2012}
}

@article{zhu2014big,
  title={Big learning with bayesian methods},
  author={Zhu, Jun and Chen, Jianfei and Hu, Wenbo},
  journal={arXiv preprint arXiv:1411.6370},
  year={2014}
}


@article{bardenet2015markov,
  title={On {Markov} chain {Monte Carlo} methods for tall data},
  author={Bardenet, R{\'e}mi and Doucet, Arnaud and Holmes, Chris},
  journal={arXiv preprint arXiv:1505.02827},
  year={2015}
}



@article{green2015bayesian,
  title={{Bayesian} computation: a summary of the current state, and samples backwards and forwards},
  author={Green, Peter J and {\L}atuszy{\'n}ski, Krzysztof and Pereyra, Marcelo and Robert, Christian P},
  journal={Statistics and Computing},
  volume={25},
  number={4},
  pages={835--862},
  year={2015},
  publisher={Springer}
}

@article{huang2005sampling,
  title={Sampling for {Bayesian} computation with large datasets},
  author={Huang, Zaijing and Gelman, Andrew},
  journal={Available at SSRN 1010107},
  year={2005}
}

@article{baker2015computational,
  title={Computational Statistics for Big Data},
  author={Baker, Jack and Fearnhead, Paul and Fox, Emily},
  year={2015}
}

@article{rabinovich2015variational,
  title={Variational consensus {Monte Carlo}},
  author={Rabinovich, Maxim and Angelino, Elaine and Jordan, Michael I},
  journal={arXiv preprint arXiv:1506.03074},
  year={2015}
}

@inproceedings{bardenet2014towards,
  title={Towards scaling up {Markov} chain {Monte Carlo}: an adaptive subsampling approach},
  author={Bardenet, R{\'e}mi and Doucet, Arnaud and Holmes, Chris},
fullbooktitle={Proceedings of the 31st International Conference on Machine Learning (ICML-14)},
booktitle = {ICML},
  pages={405--413},
  year={2014}
}


@inproceedings{firefly,
	title = {Firefly {Monte Carlo}: Exact {MCMC} with Subsets of Data},
	fullbooktitle = {Thirtieth Conference on Uncertainty in Artificial Intelligence (UAI)},
	booktitle = {UAI},	
	year = {2014},
	_month = {07/2014},		
	_author = {Dougal Maclaurin and Ryan P. Adams}
	author = {D. Maclaurin and R.P. Adams}	
}


@inproceedings{austerity,
  title={Austerity in {MCMC} Land: Cutting the {Metropolis-Hastings} Budget},
  author={Anoop Korattikara and Yutian Chen and Max Welling},
  fullbooktitle={Proceedings of the 31st International Conference on Machine Learning (ICML-14)},
    booktitle={ICML},
  _pages={405--413},
  year={2014}
}


@inproceedings{welling2011bayesian,
  title={{Bayesian} learning via stochastic gradient {Langevin} dynamics},
  _author={Welling, Max and Teh, Yee W},
    author={Welling, M. and Teh, Y.W.},
  fullbooktitle={Proceedings of the 28th International Conference on Machine Learning (ICML-11)},
  booktitle={ICML},  
  _pages={681--688},
  year={2011}
}



@article{angelino2016patterns,
  title={Patterns of Scalable {Bayesian} Inference},
  author={Elaine Angelino and Matthew James Johnson and Ryan P. Adams},
  journal={http://arxiv.org/abs/1602.05221},
  year={2015}
}


@article{zeiler2012adadelta,
  title={ADADELTA: an adaptive learning rate method},
  author={Zeiler, Matthew D},
  journal={arXiv preprint arXiv:1212.5701},
  year={2012}
}

@article{scholkopft1999fisher,
    title={Fisher discriminant analysis with kernels},
    author={Scholkopft, Bernhard and Mullert, Klaus-Robert},
    journal={Neural networks for signal processing IX},
    volume={1},
    number={1},
    pages={1},
    year={1999}
}

@inproceedings{gershman2012nonparametric,
author = {Gershman, Samuel and Hoffman, Matt and Blei, David},
title = {Nonparametric variational inference},
booktitle = { ICML},
year =  {2012}
}



@article{hoffman2013stochastic,
  title={Stochastic variational inference},
  _author={Hoffman, Matthew D and Blei, David M and Wang, Chong and Paisley, John},
  author={Hoffman, M.D. and Blei, D.M. and Wang, C. and Paisley, J.},  
  journal={JMLR},
  _volume={14},
  _number={1},
  _pages={1303--1347},
  year={2013},
  _publisher={JMLR. org}
}

@inproceedings{kucukelbir2015automatic,
  title={Automatic variational inference in stan},
  author={Kucukelbir, Alp and Ranganath, Rajesh and Gelman, Andrew and Blei, David},
  booktitle={Advances in Neural Information Processing Systems},
  pages={568--576},
  year={2015}
}

@inproceedings{kucukelbir2015automatic,
  title={Automatic variational inference in stan},
  author={Kucukelbir, Alp and Ranganath, Rajesh and Gelman, Andrew and Blei, David},
  booktitle={Advances in Neural Information Processing Systems},
  pages={568--576},
  year={2015}
}


@inproceedings{ranganath2013black,
  title={Black box variational inference},
  author={Ranganath, Rajesh and Gerrish, Sean and Blei, David M},
  booktitle={AI and Statistics},
  year={2014}
}


@inproceedings{gershman2012nonparametric,
  title={Nonparametric variational inference},
  author={Gershman, Samuel and Hoffman, Matt and Blei, David},
  booktitle={International Conference on Machine Learning},
  year={2012}
}

@inproceedings{jimenez2015variational,
  title={Variational Inference with Normalizing Flows},
  author={Danilo Jimenez Rezende and Mohamed, Shakir},
  booktitle={The 32nd International Conference on Machine Learning},
  year={2015}
}


@article{marzouk2016introduction,
  title={An introduction to sampling via measure transport},
  author={Marzouk, Youssef and Moselhy, Tarek and Parno, Matthew and Spantini, Alessio},
  journal={arXiv preprint arXiv:1602.05023},
  year={2016}
}


@inproceedings{mnih2014neural,
  title={Neural variational inference and learning in belief networks},
  author={Mnih, Andriy and Gregor, Karol},
  booktitle={ICML},
  year={2014}
}

@inproceedings{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  booktitle={ICLR},  
  _booktitle={The International Conference on Learning Representations (ICLR)},
  year={2013}
}

@inproceedings{lawrence1998approximating,
  title={Approximating posterior distributions in belief networks using mixtures},
  author={Lawrence, Christopher M Bishop Neil and Jordan, Tommi Jaakkola Michael I},
  booktitle={Advances in Neural Information Processing Systems 10: Proceedings of the 1997 Conference},
  volume={10},
  pages={416},
  year={1998},
  organization={MIT Press}
}



@phdthesis{lawrence2001variational,
  title={Variational inference in probabilistic models},
  author={Lawrence, Neil David},
  year={2001},
  school={University of Cambridge}
}


@inproceedings{jaakkola1999improving,
  title={Improving the mean field approximation via the use of mixture distributions},
  author={Jaakkola, T.S. and Jordon, M.I.},
  booktitle={Learning in graphical models},
  pages={163--173},
  year={1999},
  organization={MIT Press}
}

@inproceedings{challis2012affine,
  title={Affine independent variational inference},
  author={Challis, Edward and Barber, David},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2186--2194},
  year={2012}
}

@inproceedings{titsias2014doubly,
  title={Doubly stochastic variational Bayes for non-conjugate inference},
  author={Titsias, Michalis and L{\'a}zaro-Gredilla, Miguel},
  booktitle={Proceedings of the 31st International Conference on Machine Learning (ICML-14)},
  pages={1971--1979},
  year={2014}
}

@inproceedings{dai2016provable,
  title={Provable Bayesian Inference via Particle Mirror Descent},
  author={Bo Dai and Niao He and Hanjun Dai and Le Song},
  booktitle={AISTATS},
  _booktitle = { The 19th International Conference on Artificial Intelligence and Statistics}, 
  year={2016}
}


  @book{villani2008optimal,
  title={Optimal transport: old and new},
  author={Villani, C{\'e}dric},
  volume={338},
  year={2008},
  publisher={Springer Science \& Business Media}
}

@book{jordan1998learning,
  title={Learning in graphical models},
  author={Jordan, Michael Irwin},
  volume={89},
  year={1998},
  publisher={Springer Science \& Business Media}
}


@inproceedings{han2015variational,
  title={Variational Gaussian Copula Inference},
  author={Shaobo Han and Xuejun Liao and David B. Dunson and Lawrence Carin},
  booktitle={The 19th International Conference on Artificial Intelligence and Statistics (AISTATS)},
  year={2016},
}

@article{tran2015copula,
  title={Copula variational inference},
  author={Dustin Tran and David M. Blei and Edoardo M. Airoldi},
  journal={Neural Information Processing Systems},
  year={2015}
}


@article{duchi2011adaptive,
  title={Adaptive subgradient methods for online learning and stochastic optimization},
  author={Duchi, John and Hazan, Elad and Singer, Yoram},
  journal={The Journal of Machine Learning Research},
  volume={12},
  pages={2121--2159},
  year={2011},
  publisher={JMLR. org}
}

@book{cover2012elements,
  title={Elements of information theory},
  author={Cover, Thomas M and Thomas, Joy A},
  year={2012},
  publisher={John Wiley \& Sons}
}

@incollection{bottou2012stochastic,
  title={Stochastic gradient descent tricks},
  author={Bottou, L{\'e}on},
  booktitle={Neural Networks: Tricks of the Trade},
  pages={421--436},
  year={2012},
  publisher={Springer}
}

@article{kulkarni2014variational,
  title={Variational Particle Approximations},
  author={Kulkarni, Tejas D and Saeedi, Ardavan and Gershman, Samuel},
  journal={arXiv preprint arXiv:1402.5715},
  year={2014}
}

@article{homan2014no,
  title={The no-U-turn sampler: Adaptively setting path lengths in Hamiltonian Monte Carlo},
  author={Homan, Matthew D and Gelman, Andrew},
  journal={The Journal of Machine Learning Research},
  volume={15},
  number={1},
  pages={1593--1623},
  year={2014},
  publisher={JMLR. org}
}

@article{foreman2013emcee,
  title={emcee: the MCMC hammer},
  author={Foreman-Mackey, Daniel and Hogg, David W and Lang, Dustin and Goodman, Jonathan},
  journal={Publications of the Astronomical Society of the Pacific},
  volume={125},
  number={925},
  pages={306},
  year={2013},
  publisher={IOP Publishing}
}


@article{gal2015dropout,
  title={Dropout as a Bayesian approximation: Representing model uncertainty in deep learning},
  author={Gal, Yarin and Ghahramani, Zoubin},
  journal={arXiv preprint arXiv:1506.02142},
  year={2015}
}

@inproceedings{hernandez2015probabilistic,
  title={Probabilistic backpropagation for scalable learning of bayesian neural networks},
  author={Hern{\'a}ndez-Lobato, Jos{\'e} Miguel and Adams, Ryan P},
  booktitle={Proceedings of International Conference on Machine Learning (ICML)},
  year={2015}
}


@article{li2016variational,
  title={Variational Inference with R$\backslash$'enyi Divergence},
  author={Li, Yingzhen and Turner, Richard E},
  journal={arXiv preprint arXiv:1602.02311},
  year={2016}
}

@inproceedings{li2015stochastic,
  title={Stochastic expectation propagation},
  author={Li, Yingzhen and Hern{\'a}ndez-Lobato, Jos{\'e} Miguel and Turner, Richard E},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2314--2322},
  year={2015}
}

@article{gal2015dropout,
  title={Dropout as a Bayesian approximation: Representing model uncertainty in deep learning},
  author={Gal, Yarin and Ghahramani, Zoubin},
  journal={arXiv preprint arXiv:1506.02142},
  year={2015}
}

@misc{Bache+Lichman:2013,
author = "K. Bache and M. Lichman",
year = "2013",
title = "{UCI} Machine Learning Repository",
url = "http://archive.ics.uci.edu/ml",
institution = "University of California, Irvine, School of Information and Computer Sciences" }



@article{collobert2002parallel,
  title={A parallel mixture of {SVMs} for very large scale problems},
  author={Collobert, Ronan and Bengio, Samy and Bengio, Yoshua},
  journal={Neural computation},
  volume={14},
  number={5},
  pages={1105--1114},
  year={2002},
  publisher={MIT Press}
}


==> out <==
./appendix.tex:$$\nabla_\para \KL(q_{[T]} ~|| ~ p )  =  
./appendix.tex:%\KL(q_{[T]} ~|| ~ p ) = \KL(q ~||~ p_{- \para}), 
./appendix.tex:\KL(q_{[T]} ~|| ~ p ) = \KL(q ~||~ p_{[T^{-1}]}), 
./appendix.tex:\nabla_\para \KL(q_{[T]} ~|| ~ p )  =   - \E_{x\sim q} [\nabla_{\para} \log p_{[T^{-1}]}(x)]. 
./appendix.tex:%Taking the derivative for KL divergence gives
./appendix.tex:%\nabla_{\para}\KL(q_{[T]} ~||~ p ) %~\big|_{\para = 0} 
./appendix.tex:Define $F[f] =  \KL(q_{[x+f(x)]} ~||~ p) =
./appendix.tex: \KL(q ~||~ p_{[(x+f(x))^{-1}]} )$, we have 
./appendix.tex:& = \KL(q ~||~ p_{[(x+f(x)+\epsilon g(x))^{-1}]} )  \\
./main.tex:% based on evolving a set of particles to minimize KL divergence. %iterative transport a set of particles to the target distribution. 
./main.tex:by applying a form of functional gradient descent that minimizes the KL divergence. % of the true and the particle distributions. 
./main.tex:%Our method uses a set of particles for approximation, on which incremental transforms (in the form of a gradient descent) are applied recursively to mininimize the KL divergence between the true posterior and the distribution that the particle represents. 
./main.tex:%Instead of assuming a parametric form on the variational reference distribution, we recursively apply transforms on a set of particles  to minimize the KL divergence in the fastest direction. 
./main.tex:that connects KL divergence with a recently proposed kernelized Stein discrepancy, which is of independent interest. 
./main.tex:%Our key result is based on a generation of deBruijn identity that connects the derivative of KL divergence under smooth transform with Stein's identity. 
./main.tex:%Variational inference provides a powerful tool for addressing this difficulty, by defining a set of simple distributions in which a best approximation is found by minimizing a KL divergence criterion. 
./main.tex:%The variational inference methods provide an determinstic alternative by framing instead frame the Bayesian inference problem into an deterministic optimization problem that involves approximating the target distribution with a simpler distributions by minimizing their KL divergence. 
./main.tex:The variational inference methods instead frame the Bayesian inference problem into deterministic optimizations that approximate the target distribution with simpler distributions by minimizing their KL divergence. 
./main.tex:% KL divergence is mi
./main.tex:In this work, we propose a new general purpose variational inference algorithm which can be treated as a natural counterpart of gradient descent for full Bayesian inference. Our algorithm uses a set of particles for approximation, on which a form of (functional) gradient descent is performed to minimize the KL divergence and drive the particles to fit with the true posterior distribution. 
./main.tex:%In this work, we propose a new simple and generic variational inference algorithm that approximates the target distribution using a population of particles by minimizing their KL divergence. 
./main.tex:%Our method performs a form of collective gradient descent on the particles that gives the steepest descent on the KL divergence, which iteratively \emph{transport} a set of initial particles (e.g., drawn from the prior distribution) to the desired target posterior distribution. 
./main.tex:%which transport the probability mass of the particles toward according to the direction that decreases the KL divergence at the 
./main.tex:\todo{In this work,  we propose a new variational inference algorithm that is based on minimizing the KL divergence of a population of particles and the target distribution. 
./main.tex:We maintain a set of particles, and apply transforms sequentially to minimize KL divergence. We find a closed form solution for the optimal local transform that gives the steepest descent on the KL divergence in a kernel space. This yields a simple algorithm with a (kernelized) gradient descent. Interestingly, our algorithm automatically reduces to the typical gradient descent for penalized maximum likelihood (i.e., finding the posterior mode) with one particle (or with a kernel of zero bandwidth). This allows us provides a practical computational procedure that smooths between penalized maximum likelihood and Bayesian methods by simply adding the number of particles. Our algorithm is therefore well suited for automatic implementation. }
./main.tex:that connects the derivative of KL divergence w.r.t. smooth variable transforms and a recently introduced kernelized Stein discrepancy \citep{oates2014control,  chwialkowski2016kernel, liu2016kernelized}, 
./main.tex:that gives the steepest descent on the KL divergence
./main.tex:%functional gradient to give the steepest descent on the KL divergence within a 
./main.tex:%which allows us to derive a closed form solution for the optimal local transform within a reproducing kernel Hilbert space (RKHS) that defines the steepest descent on the KL divergence in a kernel space. 
./main.tex:%*The idea of variational inference by recursively transforming particles has been discussed in several recent work \citep{jimenez2015variational,  marzouk2016introduction}. *Our key contribution is to reveal a theoretical connection between  the derivatives of KL divergence w.r.t. smooth transforms and a recently introduced kernelized Stein discrepancy \cite{oates2014control,  chwialkowski2016kernel, liu2016kernelized}; this result extends the well known connection of derivative of KL divergence and Fisher divergence, and deBurijn identity. Using the result in \citet{liu2016kernelized}, we can find the a closed form solution for the optimal local transform that gives the steepest descent on the KL divergence in a kernel space. This close form makes our algorithm highly efficient, and ease to implement. We expect that this result will find more general application beyond variational inference. 
./main.tex:Our main results are presented in Section~\ref{sec:method} in which we clarify the connection between KSD and KL divergence, and leverage it to develop our novel variational inference method. 
./main.tex:%In this work, we will clarify the connection between KSD and KL divergence, and leverage it to develop our novel variational inference method. 
./main.tex:%We give a brief introduction on Stein's identity and the recently proposed kernelized Stein discrepancy (KSD) \citep{liu2016kernelized, oates2014control, chwialkowski2016kernel}. In this work, we will clarify the connection between KSD and KL divergence, and leverage it to develop our novel variational inference method. 
./main.tex:Variational inference approximates $p(x)$ using a simpler distribution $q(x)$ by minimizing their KL divergence. 
./main.tex:q^* = \argmin_{q \in \mathcal Q} \big\{ \KL(q ~||~ p) \equiv   \E_q \log q  - \E_q [\log \bar p(x)]  + \log Z \big\}, 
./main.tex:iii) \emph{Solvable}, so that the followed KL minimization problem can be efficiently solved.  
./main.tex:%strike a balance between the flexibility for close approximation of the target distribution as well as the computational tractability for the followed KL minimization problem. 
./main.tex:%The choice of the set $\mathcal Q$ of easy distributions forms a key component of the design of variational inference, which should strike a balance between the flexibility for close approximation of the target distribution as well as the computational tractability for the followed KL minimization problem. 
./main.tex:\subsection{Stein Operator as the Derivative of KL Divergence}\label{sec:steinKL}
./main.tex:minimize the KL divergence in \eqref{equ:kl},
./main.tex:The following result, which forms the foundation of our method, draws an insightful connection between Stein operator and the derivative of KL divergence w.r.t. the perturbation magnitude $\para$. 
./main.tex:\nabla_{\para}\KL(q_{[\T]} ~||~ p ) ~\big|_{\para = 0} =  - \E_{x\sim q} [\trace(\stein_p \ff(x))], 
./main.tex:we can identify the optimal perturbation direction that gives the steepest descent on the KL divergence in the unit ball of a RKHS. % at the fastest speed. 
./main.tex:for which the negative gradient in \eqref{equ:pdir} equals KSD, that is, $\nabla_{\para}\KL(q_{[\T]} ~||~ p ) ~\big|_{\para = 0} =-\S(q, ~ p)$. 
./main.tex:%the square root of the negative kernelized Stein discrepancy, that is, $\nabla_{\para}\KL(q_{[\T]} ~||~ p ) ~\big|_{\para = 0} =  - \sqrt{\S(p, ~ q)}$. 
./main.tex:%2. We have $$ \min_{\phi \in \H\colon ||\phi||_\H \leq 1} \bigg\{ \nabla_{\para}\KL(q_{\para\phi} ~||~ p ) ~\big|_{\para = 0}   \bigg\} =   -   \S(q_0,  ~p),$$ %\E_{x\sim q_0} [\trace(\stein \phi(x))],  and the optimal $\phi$ is obtained at %$\phi^*(\cdot) \propto $$$\phi^*(\cdot) \propto \E_{x\sim q_0}[\stein_p k(x, \cdot)]. $$
./main.tex:%Therefore, $\phi^*(x)$ defines the optimal smooth perturbation direction that decreases $\KL(q_\para ~||~p)$ at the fastest speed, 
./main.tex: the KL divergence by an amount of $\epsilon_0 \cdot \S(q_0, ~ p)$, where $\epsilon_0$ is a small step size; % of $\epsilon$; 
./main.tex: this would give a reference distribution $q_1(x) = q_{0[\T_0]}(x)$, on which a further transform $\T_1(x) = x + \epsilon_1 \cdot \ff^*_{p,q_1}(x)$ can further decrease the KL divergence by $\epsilon_1 \cdot \S(q_1, ~ p)$. 
./main.tex:%one should choose $\phi(x)$ to maximize the negative gradient $\E_{q}[\stein_p\phi(x)]$, and by applying $\T(x) = x + \epsilon \phi^*(x)$, we decrease the KL divergence by amount of $\epsilon \cdot \S(q, ~ p);$  
./main.tex:\nabla_{\vf} \KL(q_{[\T]} ~||~ p) ~ \big | _{\vf=0} = %- \E_{x\sim q}[ \nabla_x \log p(x) k(x, \cdot) + \nabla_{x} k(x, \cdot)] \equiv 
./main.tex:$$\nabla_\para \KL(q_{[\T]} ~||~ p) \big |_{\para = 0} = - \F(q, ~ p),$$
./main.tex:Note that this can be treated as a deterministic version of \emph{de Bruijn's identity} \citep{cover2012elements, lyu2009interpretation}, which draws similar connection between KL and Fisher divergence, but uses randomized linear transform $\T(x) = x+ \sqrt{\epsilon} \cdot \xi$, where $\xi$ is a standard Gaussian noise.  % with variance $\epsilon$. 
./main.tex:%$\nabla_\para \KL(q_{[\T]} ~||~ p) = $ 
./main.tex:$\ell$ a predefined length; %, and optimizes the parameters to minimize the variational KL divergence; 
./main.tex:Optimizing such mixture KL objectives often requires certain approximation, 
./main.tex:%Highly related to our work is the Gaussian mixture variational inference, which however experiments difficulty in calculating the KL objective \citep{lawrence1998approximating, jaakkola1999improving, lawrence2001variational}; this was recently done by approximating the entropy using Jensen's inequality and the expectation term using Taylor approximation \citep{gershman2012nonparametric}. 
./main.tex:%   \includegraphics[height=.15\textwidth, trim={0cm 0 0 0}, clip]{figures/0iter_KLtransport_1DGauss} &
./main.tex:%   \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/10iter_KLtransport_1DGauss} &
./main.tex:%   \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/20iter_KLtransport_1DGauss} &
./main.tex:  % \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/50iter_KLtransport_1DGauss} &
./main.tex:%   \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/100iter_KLtransport_1DGauss}  &
./main.tex:%   \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/1000iter_KLtransport_1DGauss}        \\
./main.tex:   \includegraphics[height=.15\textwidth, trim={0cm 0 0 0}, clip]{figures/0iter_KLtransport_1DGaussm1n10m2n2_2_2} &
./main.tex:%   \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/25iter_KLtransport_1DGaussm1n10m2n2_2_2}       &   
./main.tex:   \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/50iter_KLtransport_1DGaussm1n10m2n2_2_2} &
./main.tex:   \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/75iter_KLtransport_1DGaussm1n10m2n2_2_2} &
./main.tex:   \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/100iter_KLtransport_1DGaussm1n10m2n2_2_2} &
./main.tex:   \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/150iter_KLtransport_1DGaussm1n10m2n2_2_2}  &   
./main.tex:   \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/500iter_KLtransport_1DGaussm1n10m2n2_2_2}  
./main.tex:   \includegraphics[height=.15\textwidth, trim={0cm 0 0 0}, clip]{figures/x_KLtranspVaryN_m1n10m2n2_2_2NVec10_10_1000} &
./main.tex:   \includegraphics[height=.15\textwidth, trim={1.4cm 0 0 0}, clip]{figures/x2_KLtranspVaryN_m1n10m2n2_2_2NVec10_10_1000} &
./main.tex:   \includegraphics[height=.15\textwidth, trim={1.99cm 0 0 0}, clip]{figures/cos_KLtranspVaryN_m1n10m2n2_2_2NVec10_10_1000} &
./main.tex:%Our main theoretical findings reveals the connection between KL divergence and kernelized Stein discrepancy, which has its own independent interest. 
./main.tex:Future directions include more theoretical understanding on our method, and other potential applications of our basic Theorem in Section~\ref{sec:steinKL}. 
./main.tex:%our main theoretical findings reveals the connection between KL divergence and kernelized Stein discrepancy, which has its own independent interest. 

